Fooling Yourself: how narratives shape beliefs

Narratives often combine diagnostic evidence with truthful but nondiagnostic details. In a two-state experiment with known signal likelihoods, we test whether such details distort belief updating. Although Bayes' rule prescribes no revision, nondiagnostic signals induce revisions consistent with considering both states equally likely. Such revisions are most frequent when nondiagnostic signals appear as clues in a story, less frequent in an abstract urn problem, and virtually absent when the same story replaces these clues with explicit no-information messages. Simulations show that these revisions reduce belief accuracy and delay decisions, an effect communicators could exploit without lying.

==> Tables/reg_toward_midpoint.tex <==
\begin{table}[H]\centering
\caption{Movement toward uncertainty.}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{cc}}
\hline\hline
  $M$  &  & \\
\hline             
\textit{Urn}  &0.039\sym{\dagger} (0.02)         \\
\textit{Story No Info}       &0.004 (0.02)         \\
$d_{t-1}$    &0.554\sym{***} (0.05)         \\
\textit{Urn} $\times d_{t-1}$ &-0.222\sym{**} (0.07)         \\
\textit{Story No Info} $\times d_{t-1}$ &-0.284\sym{***} (0.08)         \\
Constant   &-0.058\sym{**} (0.02)         \\
\hline
Observations&  784 \\
\hline\hline
\end{tabular}
\caption*{\footnotesize\textit{Notes:} Movement toward uncertainty after receiving a nondiagnostic signal. The table reports results from a mixed-effect model, controlling for round fixed effects, the strength of evidence received up to time $t$, and allowing for subject-level intercepts. Standard errors in parentheses. \footnotesize \sym{\dagger} \(p<0.10\), \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)\label{tab:probability_midpoint}}
\end{table}

